Source mass characterization in the ARIADNE axion experiment

The Axion Resonant InterAction Detection Experiment (ARIADNE) is a collaborative effort to search for the QCD axion using nuclear magnetic resonance (NMR), where the axion acts as a mediator of spin-dependent forces between an unpolarized tungsten source mass and a sample of polarized helium-3 gas. Since the experiment involves precision measurement of a small magnetization, it relies on limiting ordinary magnetic noise with superconducting magnetic shielding. In addition to the shielding, proper characterization of the noise level from other sources is crucial. We investigate one such noise source in detail: the magnetic noise due to impurities and Johnson noise in the tungsten source mass.

==> bib.tex <==
\begin{thebibliography}{99}

\bibitem{minaandy} A. Arvanitaki and A. Geraci, Phys. Rev. Lett. {\bf{113}}, 161801 (2014).

\bibitem{axion}
%\cite{Peccei:1977hh}
  R.~D.~Peccei and H.~R.~Quinn,
  %``CP Conservation in the Presence of Instantons,''
  Phys.\ Rev.\ Lett.\  {\bf 38}, 1440 (1977);
  %\cite{Weinberg:1977ma}
  S.~Weinberg,
  %``A New Light Boson?,''
  Phys.\ Rev.\ Lett.\  {\bf 40}, 223 (1978);
  %\cite{Wilczek:1977pj}
  F.~Wilczek,
  %``Problem of Strong p and t Invariance in the Presence of Instantons,''
  Phys.\ Rev.\ Lett.\  {\bf 40}, 279 (1978).
  %\cite{Dimopoulos:2008sv}

  %\cite{Moody:1984ba}
\bibitem{Moody:1984ba}
  J.~E.~Moody and F.~Wilczek,
  Phys.\ Rev.\ D {\bf 30}, 130 (1984).
%  \bibitem{bicep2} P.A.R. Ade {\it{et. al.}} (BICEP2 Collaboration) Phys. Rev. Lett. {\bf{112}}, 241101 (2014).


%\bibitem{Svrcek:2006yi}
  P.~Svrcek and E.~Witten,
  JHEP {\bf 0606}, 051 (2006)
  [hep-th/0605206].

\bibitem{axiverse}
A. Arvanitaki, S. Dimopoulos, S. Dubovsky, N. Kaloper, J. March-Russell, Phys. Rev. D {\bf{81}},123530 (2010).

\bibitem{PDG}
  J.~Beringer {\it et al.}  [Particle Data Group Collaboration],
  ``Review of Particle Physics (RPP),''
  Phys.\ Rev.\ D {\bf 86}, 010001 (2012).

  \bibitem{axionCDM} L. Visinelli and P. Gondolo,  Phys. Rev. Lett {\bf{113}} 011802 (2014).

 \bibitem{axionCDM2} David J. E. Marsh, Daniel Grin, Renée Hlozek, and Pedro G. Ferreira, Phys. Rev. Lett. {\bf{113}}, 011801 (2014).

\bibitem{BH1}
A. Arvanitaki, S. Dubovsky, Phys.Rev. D {\bf{83}}, 044026 (2011).
\bibitem{BH2}
A. Arvanitaki, M. Baryakhtar, X. Huang, Phys.Rev. D91, 084011 (2015). 


\bibitem{ADMX} S. J. Asztalos, G. Carosi, C. Hagmann, D. Kinion, K. van Bibber, M. Hotz, L. J Rosenberg, G. Rybka, J. Hoskins, J. Hwang, P. Sikivie, D. B. Tanner, R. Bradley, and J. Clarke, Phys. Rev. Lett. {\bf{104}} 041301 (2010).

%\bibitem{scalaraxioncoupling}
%\cite{Pospelov:1997uv}
%\bibitem{Pospelov:1997uv}
%  M.~Pospelov,
%  ``CP odd interaction of axion with matter,''
%  Phys.\ Rev.\ D {\bf 58}, 097703 (1998)
%  [hep-ph/9707431];
  %%CITATION = HEP-PH/9707431;%%
  %17 citations counted in INSPIRE as of 13 Feb 2014
%  M.~Pospelov,
%  ``Best values for the CP odd meson nucleon couplings from supersymmetry,''
%  Phys.\ Lett.\ B {\bf 530}, 123 (2002)
%  [hep-ph/0109044];
  %%CITATION = HEP-PH/0109044;%%
  %31 citations counted in INSPIRE as of 13 Feb 2014
  %\cite{Pospelov:2005pr}
%\bibitem{Pospelov:2005pr}
%  M.~Pospelov and A.~Ritz,
%  ``Electric dipole moments as probes of new physics,''
%  Annals Phys.\  {\bf 318}, 119 (2005)
%  [hep-ph/0504231].
  %%CITATION = HEP-PH/0504231;%%
  %287 citations counted in INSPIRE as of 13 Feb 2014


%\bibitem{giovanniaxion}
%G. G. di Cortona, E. Hardy, J. P. Vegaa, and G. Villadoro, ``The QCD axion, precisely'', Journal of High Energy Physics 2016:34 (2016).


\bibitem{Raffelt:2012sp}
  G.~Raffelt,
 % ``Limits on a CP-violating scalar axion-nucleon interaction,''
  Phys.\ Rev.\ D {\bf 86}, 015001 (2012).
  %%CITATION = ARXIV:1205.1776;%%
  %7 citations counted in INSPIRE as of 11 Oct 2013

  %\cite{Vasilakis:2008yn}
\bibitem{Vasilakis:2008yn}
  G.~Vasilakis, J.~M.~Brown, T.~W.~Kornack and M.~V.~Romalis,
  %``Limits on new long range nuclear spin-dependent forces set with a K - He-3 co-magnetometer'',
Phys.\ Rev.\ Lett.\  {\bf 103}, 261801 (2009).
  %%CITATION = ARXIV:0809.4700;%%
  %19 citations counted in INSPIRE as of 12 Oct 2013

%\cite{gsgpgermany}
\bibitem{gsgpgermany}
K. Tullney, F. Allmendinger, M. Burghoff, W. Heil, S. Karpuk, W. Kilian, S. Knappe-Grüneberg, W. Müller, U. Schmidt, A. Schnabel, F. Seifert, Yu. Sobolev, and L. Trahms, 
 Phys.\ Rev.\ Lett.\  {\bf 111}, 100801 (2013)

 %\cite{snow}
 \bibitem{snow}
 P.-H. Chu, A. Dennis, C. B. Fu, H. Gao, R. Khatiwada, G. Laskaris, K. Li, E. Smith, W. M. Snow, H. Yan, and W. Zheng, Phys. Rev. D {\bf{87}}, 011105(R) (2013).

 \bibitem{snow2} M. Bulatowicz, R. Griffith, M. Larsen, J. Mirijanian, C. B. Fu, E. Smith, W. M. Snow, H. Yan, and T. G. Walker,  Phys. Rev. Lett. {\bf{111}}, 102001 (2013).

\bibitem{lamoreauxhunter} A. N. Youdin, D. Krause, Jr., K. Jagannathan, L. R. Hunter, and S. K. Lamoreaux,  Phys. Rev. Lett. {\bf{77}}, 2170 (1996).

%\bibitem{PDG}
%  J.~Beringer {\it et al.}  [Particle Data Group Collaboration],
%  ``Review of Particle Physics (RPP),''
%  Phys.\ Rev.\ D {\bf 86}, 010001 (2012).

%\cite{Raffelt:2012sp}

%  \bibitem{3He}
%  J.L. Flowers, B. W. Petley and M. G. Richards, ``A Measurement of the Nuclear Magnetic Moment of the Helium-3 Atom in Terms of that of the Proton,'' Metrologia, 30, 75 (1993).

%  \bibitem{3He2}
%T. Ino and S. Muto, ``Measurements of the 3He spin relaxation below room temperature,'' Physica B, 397, 184 (2007).  R.H. Romer, ``Nuclear Spin Relaxation in Liquid He 3 II,'' Phys. Rev. 117, 1183 (1960).


%\bibitem{KSVZ} Kim, J.E. ``Weak-Interaction Singlet and Strong CP Invariance''. Phys. Rev. Lett. 43, 103 (1979), Shifman, M., Vainshtein, A., Zakharov, V.  ``Can confinement ensure natural CP invariance of strong interactions?''. Nucl. Phys. B166, 493 (1980).
%\bibitem{DFSZ} Dine, M., Fischler, W., Srednicki, M.  ``A simple solution to the strong CP problem with a harmless axion'', Phys. Lett. B104, 199 (1981),  Zhitnitsky, A.  ``On possible suppression of the axion-hadron interactions''. Sov. J. Nucl. Phys. 31, 260 (1980).

\bibitem{x3} K. van Bibber and G. Carosi, 8th Patras Workshop on Axions, WIMPs, and WISPs, Chicago, IL, July 18-22, arxiv: 1304.7803 (2012).

\bibitem{orpheus} G. Rybka, A. Wagner, K. Patel, R. Percival, K. Ramos, and A. Brill, Phys. Rev. D {\bf{91}}, 011701(R) (2015).
\bibitem{LCcircuits} B. Cabrera and S. Thomas, Workshop Axions 2010, U. Florida, 2010.

  \bibitem{casper}
  D.~Budker, P.~W.~Graham, M.~Ledbetter, S.~Rajendran and A.~Sushkov,
  Phys. Rev. X {\bf{4}}, 021030 (2014).


%\bibitem{Svrcek:2006yi}
%  P.~Svrcek and E.~Witten,
%  ``Axions In String Theory,''
%  JHEP {\bf 0606}, 051 (2006)
%  [hep-th/0605206].
  %%CITATION = HEP-TH/0605206;%%
  %238 citations counted in INSPIRE as of 13 Feb 2014

%\bibitem{axiverse}
  %\cite{Arvanitaki:2009fg}
%  Asimina Arvanitaki, Savas Dimopoulos, Sergei Dubovsky, Nemanja Kaloper, and John March-Russell,
%  ``String Axiverse,''
%  Phys.\ Rev.\ D {\bf 81}, 123530 (2010);



%  \bibitem{raffelt2008} G. G. Raffelt, Lect. Notes Phys. 741, 51 (2008).

%  \bibitem{BH}
  %%CITATION = ARXIV:0905.4720;%%
%  A. Arvanitaki and S. Dubovsky, ``Exploring the string axiverse with precision black hole physics'', Phys.Rev.\textbf{D 83}, 044026 (2011).

%  \bibitem{bicep2} P.A.R. Ade {\it{et. al.}} (BICEP2 Collaboration) Phys. Rev. Lett. {\bf{112}}, 241101 (2014).

%  \bibitem{axionCDM} L. Visinelli and P. Gondolo, ``Axion cold dark matter in view of BICEP2 results'', Phys. Rev. Lett {\bf{113}} 011802 (2014).


%  \bibitem{ADMX} S. J. Asztalos, G. Carosi, C. Hagmann, D. Kinion, K. van Bibber, M. Hotz, L. J Rosenberg, G. Rybka, J. Hoskins, J. Hwang, P. Sikivie, D. B. Tanner, R. Bradley, and J. Clarke, ``SQUID-Based Microwave Cavity Search for Dark-Matter Axions'' Phys. Rev. Lett. {\bf{104}} 041301 (2010).


  %\cite{Vasilakis:2008yn}
%\bibitem{Vasilakis:2008yn}
%  G.~Vasilakis, J.~M.~Brown, T.~W.~Kornack and M.~V.~Romalis,
%  ``Limits on new long range nuclear spin-dependent forces set with a K - He-3 co-magnetometer'',
%Phys.\ Rev.\ Lett.\  {\bf 103}, 261801 (2009).
  %%CITATION = ARXIV:0809.4700;%%
  %19 citations counted in INSPIRE as of 12 Oct 2013

%\cite{gsgpgermany}
%\bibitem{gsgpgermany}
%K. Tullney, F. Allmendinger, M. Burghoff, W. Heil, S. Karpuk, W. Kilian, S. Knappe-Grüneberg, W. Müller, U. Schmidt, A. Schnabel, F. Seifert, Yu. Sobolev, and L. Trahms, ``Constraints on Spin-Dependent Short-Range Interaction between Nucleons''
% Phys.\ Rev.\ Lett.\  {\bf 111}, 100801 (2013)

 %\cite{snow}
% \bibitem{snow}
% P.-H. Chu, A. Dennis, C. B. Fu, H. Gao, R. Khatiwada, G. Laskaris, K. Li, E. Smith, W. M. Snow, H. Yan, and W. Zheng, ``Laboratory search for spin-dependent short-range force from axionlike particles using optically polarized 3He gas'' Phys. Rev. {\bf{D 87}}, 011105(R) (2013).

 %\bibitem{snow2} M. Bulatowicz, R. Griffith, M. Larsen, J. Mirijanian, C. B. Fu, E. Smith, W. M. Snow, H. Yan, and T. G. Walker, ``Laboratory Search for a Long-Range T -Odd, P -Odd Interaction from Axionlike Particles Using Dual-Species Nuclear Magnetic Resonance with Polarized Xe 129 and Xe 131 Gas'' Phys. Rev. Lett. 111, 102001 (2013).


%\cite{Raffelt:2012sp}
%\bibitem{Raffelt:2012sp}
%  G.~Raffelt,
%  ``Limits on a CP-violating scalar axion-nucleon interaction,''
%  Phys.\ Rev.\ D {\bf 86}, 015001 (2012).
  %%CITATION = ARXIV:1205.1776;%%
  %7 citations counted in INSPIRE as of 11 Oct 2013
%\bibitem{minaandy} A. Arvanitaki and A. Geraci,``Resonant detection of axion-mediated forces using Nuclear Magnetic Resonance'', arxiv:1403.1290 (2014).

%  \bibitem{stanford}
%  A. A. Geraci, S. J. Smullin, D. M. Weld, J. Chiaverini, and A. Kapitulnik, ``Improved constraints on non-Newtonian forces at 10 microns,'' Phys. Rev. D 78, 022002 (2008).
%  \bibitem{adelberger}
%  D. J. Kapner, T. S. Cook, E. G. Adelberger, J. H. Gundlach, B. R. Heckel, C. D. Hoyle, and H. E. Swanson, ``Tests of the Gravitational Inverse-Square Law below the Dark-Energy Length Scale,'' Phys. Rev. Lett. 98, 021101 (2007).
%  \bibitem{price}
%  J. C. Long, H. W. Chan, A. B. Churnside, E. A. Gulbis, M. C. M. Varney, and  J. C. Price, ``Upper limits to submillimetre-range forces from extra space-time dimensions,'' Nature 421, 922 (2003).



  %\cite{Budker:2013hfa}
%\bibitem{casper}
%  D.~Budker, P.~W.~Graham, M.~Ledbetter, S.~Rajendran and A.~Sushkov,
%  ``Cosmic Axion Spin Precession Experiment (CASPEr),''
%  Phys. Rev. X 4, 021030 (2014).
  %%CITATION = ARXIV:1306.6089;%%
  %11 citations counted in INSPIRE as of 13 Feb 2014

  %\cite{Pospelov:2001ys}


  %\cite{Beringer:1900zz}

  %%CITATION = PHRVA,D86,010001;%%
  %3179 citations counted in INSPIRE as of 13 Feb 2014

 % \bibitem{edmvs5thf} Sonny Mantry, Mario Pitschmann, Michael J. Ramsey-Musolf, ``Distinguishing axions from generic light scalars using EDM and fifth-force experiments'', arxiv:1401.7339 (2014).

\bibitem{midwesttungsten} material certification,  Midwest Tungsten Service, www.tungsten.com

\bibitem{precisionglass} private communication, Ron Bihler, Precision Glass Blowing, www.precisionglassblowing.com

\bibitem{ellipsoid} M. Tejedor, H. Rubio, L. Elbaile, and R. Iglesias, IEEE Trans. Magnetics, {\bf{31}}, 830 (1995).

%\bibitem{CNM2} Center for Nanomanufacturing 2, UC Davis, cnm2.engineering.ucdavis.edu

\bibitem{varpula} T. Varpula and T. Poutanen, J. Appl. Phys. {\bf{55}}, 4015 (1984).
 
  \bibitem{fukoku} Fukoku-Shinsei Corporation, 2016.

 \bibitem{direct} Aerotech Corporation, www.aerotech.com

\bibitem{snowrsi} D. S. Hussey, D. R. Rich, A. S. Belov, X. Tong, H. Yang, C. Bailey, C. D. Keith, J. Hartfield, G. D. R. Hall, T. C. Black, W. M. Snow, T. R. Gentile, W. C. Chen, G. L. Jones, and E. Wildman, Rev. Sci. Inst. {\bf{76}}, 053503 (2005).
 \bibitem{tong} T. Tong, private communication.
\bibitem{beck} D. Beck, private communication.
%\bibitem{Larat:1990} C. Larat, M. Leduc, P.J. Nacher, G. Tastevin, and G. Vermeulen, ``Heat Conduction in Spin-Polarized Gaseous 3He at Low Temperature,'' J. Low Temp. Phys. {\bf 80}, 299 (1990).

%\bibitem{tullney1} K. Tullney, F. Allmendinger, M. Burghoff, W. Heil, S. Karpuk, W. Kilian, S. Knappe-Grüneberg, W. Müller, U. Schmidt, A. Schnabel, F. Seifert, Yu. Sobolev, and L. Trahms, ``Constraints on Spin-Dependent Short-Range Interaction between Nucleons'', Phys. Rev. Lett. 111, 100801 (2013).

%\bibitem{tullney2} F. Allmendinger, W. Heil, S. Karpuk, W. Kilian, A. Scharth,
U. Schmidt, A. Schnabel, Yu. Sobolev, and K. Tullney, arxiv:1312.3225 (2013).

%\bibitem{Nacher:1991} P. J. Nacher and J. P. Dupont-Roc, ``Experimental evidence for nonwetting with superfluid helium,'' Phys Rev. Lett. {\bf 67}, 2966 (1991).
%\bibitem{Tastevin:1992} G. Tastevin, ``Investigation of Adsorption and Wetting of 3He on Cesium and Cesiated Glass,'' J. Low Temp. Phys. {\bf 89}, 669 (1992).

%\bibitem{Heil:1999} W. Heil, J. Dreyer, D. Hofmann, H. Humblot, E. Lelievre-Berna, F. Tasset, ``3He neutron spin-filter'', Physica B: Condensed Matter {\bf 267-268}, 328 (1999).
%\bibitem{Deninger:2006} A. Deninger, W. Heil, E. W. Otten, M. Wolf, R. K. Kremer, and A. Simon, ``Paramagnetic relaxation of spin polarized 3He at coated glass walls'', Eur. Phys. J. D {\bf 38} 439 (2006).

%\bibitem{nacher34mix} Marc Himbert, Jacques Dupont-Roc, Michèle Leduc and Pierre-Jean Nacher, ``Measurement of Spin-Diffusion Coefficient in Gaseous Helium between 2 K and 0.5 K '', Jpn. J. Appl. Phys. 26 211 (1987).

%\bibitem{Taber: 1978} M. A. Taber, ``Nuclear relaxation of polarized 3He diluted by liquid 4He at 4K in low magnetic fields,'' J. Phys. Colloque {\bf C6}, 192 (1978).
%\bibitem{Romer:1959} R. H. Romer, ``Nuclear Spin Relaxation in Liquid He 3,'' Phys. Rev. {\bf 115}, 1415 (1959).

%\bibitem{Nacher:1984} P. J. Nacher, G. Tastevin, M. Leduc, S. B. Crampton, and F. Laloe, ``Spin rotation effects and spin waves in gaseous 3He'', J. Physique Lett. {\bf 45}, 441 (1984).





%  \bibitem{shields} J. R. Claycomb and J. H. Miller, Jr., Rev. Sci. Inst. 70, 4562 (1999).

%\bibitem{diffusion} M. Himbert, J. Dupont-Roc, and C. Lhuillier, ``Spin-diffusion coefficient in gaseous helium between 1 and 0.5 K'', Phys. Rev. {\bf{A 39}} 6170 (1989).



%\bibitem{Gully:1984} W. J. Gully and W. J. Mullin, ``Observation of Spin Rotation Effects in Polarized He3-He4 Mixtures'', Phys. Rev. Lett. {\bf 52}, 1810 (1984).

%\bibitem{Leggett:1970} A. J. Leggett,  J. Phys. C {\bf 12}, 448 %(1970); A. J. Leggett and M. J. Rice, Phys. Rev. Lett. {\bf 20} %(1968) 586 ; erratum Phys. Rev. {\bf 21}, 506.

%\bibitem{Lhuillier:1982} C. Lhuillier and F. J.  C., Laloe, ``Transport properties in a spin polarized gas (II),'' J.  Physique {\bf 43}, 225(1982); C. Lhuillier and F. J. Laloe, ``Transport properties in a spin polarized gas (I)'' J. Physique {\bf 43}, 197(1982); C. Lhuillier, ``Transport properties in a spin polarized gas, III,''J. Physique {\bf 44}, 1 (1983).

%\bibitem{Piechon:2009} F. Piechon, J. N. Fuchs, and F. Laloe, ``Cumulative Identical Spin Rotation Effects in Collisionless Trapped Atomic Gases,'' Phys. Rev. Lett. {\bf 102}, 215301 (2009).

%\bibitem{Hayden:2007} M. E. Hayden, E. Baudin, G. Tastevin, and P. J. Nacher, ``NMR Time Reversal as a Probe of Incipient Turbulent Spin Dynamics,'' Phys. Rev. Lett. {\bf 99}, 137602 (2007).

%\bibitem{Ledbetter:2002} M. P. Ledbetter and M.V. Romalis, ``Nonlinear Effects from Dipolar Interactions in Hyperpolarized Liquid Xe 129'', Phys. Rev. Lett. {\bf 89}, 287601 (2002).

%\bibitem{Xe-spin-echo}
 % M.P. Ledbetter, I.M. Savukov, and M.V. Romalis, ``Nonlinear Amplification of Small Spin Precession Using Long-Range Dipolar Interactions'', Phys. Rev. Lett., {\bf 94}, 060801 (2005)

%\bibitem{dipolar} R. Chapman and M. G. Richards, ``Longitudinal Spin Relaxation in He3 Gas at 4.2 K'', Phys. Rev. Lett. 33, 18, (1974).

%\bibitem{nacher} Emmanuel Baudin, Michael E. Hayden, Geneviève Tastevin, Pierre-Jean Nacher, ``Nonlinear NMR dynamics in hyperpolarized liquid 3He'', C. R. Chim. (2007), doi:10.1016/j.crci.2007.07.005. arXiv:0710.3567.
%\bibitem{mixture} M.A. Taber, ``Nuclear relaxation of polarized 3He diluted by liquid 4He at 4K in low magnetic fields'', Journal de Physique, C6-192 (1978).
%\bibitem{cscoat} G. Tastevin, Journal of Low Temp Physics 89, 669 (1992)
%\bibitem{romalis} M.V.Romalis and M.P.Ledbetter, ``Transverse Spin Relaxation in Liquid Xe 129 in the Presence of Large Dipolar Fields,'' Phys. Rev. Lett. 87, 067601 (2001).

%\bibitem{ledbetter-thesis} Micah Ledbetter, ``Progress Toward a Search for a Permanent Electric Dipole Moment in Liquid 129Xe'',Ph.D. Thesis, Princeton University (2005).

%\bibitem{Fabian-priv} Fabian Allmendinger, private communication.

  \bibitem{blas-pinningforce}
George S. Park, Charles E. Cunningham, Blas Cabrera, and Martin E. Huber,
Phys.\ Rev.\ Lett. {\bf 68}, 1920 (1992).

\bibitem{simanek-vortexmass}
E.~Simanek,
%``Quantum dynamics of vortices in superconducting layers. Role of fermion bound states ''
Phys.\ Lett.\ A {\bf 194}, 4, p. 323 - 330 (1994);
L.~Janson
%``Undergraduate experiment in superconductor point-contact spectroscopy with a Nb/Au junction''
American Journal of Physics, {\bf 80}, 2, p. 133-140 (2012).

\bibitem{cryoperm} Amuneal Manufacturing Corp. www.amuneal.com

\bibitem{barnett} S. J. Barnett, Phys. Rev. {\bf 6}, 239 (1915).

%\bibitem{blastungsten} B. A. Young, T. Saab, B. Cabrera, J. J. Cross, R.M.Clarke, and R.A. Abusaidi, ``Measurement of Tc suppression in tungsten using magnetic impurities,'' Journal of Applied Physics 86, 6975 (1999)

\bibitem{patch} C. C. Speake and C. Trenkel, Phys. Rev. Lett. {\bf{90}}, 160403 (2003).

%\bibitem{stp1} Weigang Wang and Malcolm R. Beasley, ``Local sheet conductivity and sheet current density mapping using a single scanning voltage probe'', arxiv: 1309.4540 (2013).

%\bibitem{stp2} Weigang Wang, Ko Munakata, Michael Rozler, and Malcolm R. Beasley, ``Local transport measurements at mesoscopic length scales using scanning tunneling potentiometry'', Phys. Rev. Lett. 110, 236802 (2013).


\bibitem{patch2} R. O. Behunin, D. A. R. Dalvit, R. S. Decca, and C. C. Speake, arxiv: 1304.4074 (2013).

%\bibitem{japanese} T. Ino and S. Muto, Physica B 397, 182 (2007).

%\bibitem{blas-thesis} Cabrera B., Ph.D. Thesis Stanford Univ., CA (1975).

\bibitem{MPMS} Magnetic Property Measurement System, Quantum Design, Inc., http://www.qdusa.com

\bibitem{RSIinprep} H. Fosbinder-Elkins, J. Dargert, A.A. Geraci, in preparation

\bibitem{ALPS} Robin Bahre et. al., Any Light Particle Search II Technical Design Report, arxiv:1302.5647 (2013).

%\bibitem{jonathancryo} Mei-Ju Lu and Jonathan D. Weinstein, ``Cold TiO (X Δ3)-He collisions,''  New Journal of Physics 11, 055015 (2009), Naima Tariq, Nada Al Taisan, Vijay Singh, and Jonathan D. Weinstein, ``Spectroscopic Detection of the LiHe Molecule,'' Phys. Rev. Lett. 110, 153201 (2013).

%\bibitem{kapner} D. J. Kapner, T. S. Cook, E. G. Adelberger, J. H. Gundlach, B. R. Heckel, C. D. Hoyle, and H. E. Swanson, ``Tests of the Gravitational Inverse-Square Law below the Dark-Energy Length Scale'', Phys. Rev. Lett. 98, 021101 (2007).
%\bibitem{stanford}
  %A. A. Geraci, S. J. Smullin, D. M. Weld, J. Chiaverini, and A. Kapitulnik, ``Improved constraints on non-Newtonian forces at 10 microns,'' Phys. Rev. D 78, 022002 (2008), D.M. Weld, J. Xia, B. Cabrera, and A. Kapitulnik, ``New apparatus for detecting micron-scale deviations from Newtonian gravity'', Phys. Rev. D 77, 062006 (2008).
  %\bibitem{price}
  %J. C. Long, H. W. Chan, A. B. Churnside, E. A. Gulbis, M. C. M. Varney, and  J. C. Price, ``Upper limits to submillimetre-range forces from extra space-time dimensions,'' Nature 421, 922 (2003).
  
\bibitem{proceed2} A.A. Geraci, H. Fosbinder-Elkins, C. Lohmeyer, J. Dargert, M. Cunningham, M. Harkness, E. Levenson-Falk, S. Mumford, A. Kapitulnik, A. Arvanitaki, I. Lee, E. Smith, E. Wiesman, J. Shortino, J.C. Long, W.M. Snow, C.-Y. Liu, Y. Shin, Y.Semertzidis, Y.-H. Lee,  Proceedings of the 2nd Axion Cavity and Detector Workshop, 	arXiv:1710.05413 (2017). 


\bibitem{shielding}H. Fosbinder-Elkins, J. Dargert, M. Harkness, A.A. Geraci, E. Levenson-Falk, S. Mumford, A. Kapitulnik, Y. Shin, Y. Semertzidis, Y.-H.Lee, arXiv:1710.08102 (2017). 

\end{thebibliography}
